Surveys of the Galactic Center and the Nature of the Galactic Center Lobe

The Galactic center (GC) is a dense and chaotic region filled with unusual sources, such as intense star forming regions, dense star clusters, nonthermal radio filaments, and a massive black hole. The proximity of the GC region makes it an ideal place to study the unusual processes that tend to manifest themselves in Galactic nuclei. This thesis uses single-dish and interferometric radio continuum, radio recombination line, polarized radio continuum, and mid-IR observations to study the wide variety of physical processes seen in the GC region on physical scales from 0.1 to 100 parsecs. These observations provide one of the most sensitive studies of the radio continuum emission in the central 500 parsecs. I also study the properties of nonthermal radio filaments, which can constrain their origin and the structure of the magnetic field in the GC region. The presence of massive star clusters and a massive black hole suggest that starburst and AGN phenomena can manifest themselves in our Galaxy. This thesis explores this possibility by studying a 150-pc-tall, shell-like structure called the Galactic center lobe (GCL). Our observations examine the spectral index, dust emission, polarized continuum emission, and ionized gas throughout the GCL. I find strong evidence supporting the idea that the GCL is a true three-dimensional shell located in the GC region with nested layers of ionized, magnetized, and mid-IR--emitting components. I compare the physical conditions of the GCL to proposed models for its origin and find best agreement with starburst outflows seen in other galaxies, yet consistent with the currently observed pressure and star formation rate in the central tens of parsecs of our Galaxy. (abridged)

==> thesis_astro-ph.bbl.tex <==
\begin{thebibliography}{}\setlength{\itemsep}{2mm}

\bibitem[Afflerbach et al.(1996)]{a96} Afflerbach, A. Churchwell, E., Acord, J. M., Hofner, P., Kurtz, S., \& Dupree, C. G. 1996, ApJS, 106, 423

\bibitem[Aharonian et al.(2006)]{a06} Aharonian, F., et al. 2006, Nature, 439, 695

\bibitem[Allamandola et al.(1989)]{a89} Allmandola, L. J., Tielens, A. G. G. M., \& Barker, J. R. 1989, ApJS, 71, 733

\bibitem[Altenhoff et al.(1979)]{a79} Altenhoff, W. J., Downes, D., Pauls, T., \& Schraml, J. 1979, A\&AS, 35, 23

\bibitem[Anish Roshi \& Anantharamaiah(1997)]{a97} Anish Roshi, D. \& Anantharamaiah, K. R. 1997, MNRAS, 292, 63

\bibitem[Argon et al.(2000)]{a00} Argon, A. L., Reid, M. J., \& Menten, K. M. 2000, ApJS, 129, 159

\bibitem[Bajaja \& van Albada(1979)]{b79} Bajaja, E. \& van Albada, G. D. 1979, A\&A, 75, 251

\bibitem[Balick \& Brown(1974)]{b74} Balick, B. \& Brown, R. L. 1974, ApJ, 194, 265

\bibitem[Balick \& Sanders(1974)]{ba74} Balick, B. \& Sanders, R. H. 1974, ApJ, 192, 325

\bibitem[Bally(1996)]{b96} Bally, J. 1996, ASPC, 102, 8

\bibitem[Bally et al.(1987)]{b87} Bally, J., Stark, A. A., Wilson, R. W., \& Henkel, C. 1987, ApJS, 65, 13

\bibitem[Bally \& Yusef-Zadeh(1989)]{b89} Bally, J. \& Yusef-Zadeh, F. 1989, ApJ, 336, 173

\bibitem[Beck(2001)]{b01} Beck, R. 2001, SSRv, 99, 243

\bibitem[Beck \& Krause(2005)]{b05} Beck, R. \& Krause, M. 2005, AN, 326, 414

\bibitem[Becker \& Helfand(1985)]{b85} Becker, R. H. \& Helfand, D. J. 1985, Nature, 313, 115

\bibitem[Becker et al.(1994)]{b94} Becker, R. H., White, R. L., Helfand, D. J., \& Zoonematkermani, S. 1994 ApJS, 91, 347

\bibitem[Belmont et al.(2005)]{be05} Belmont, R., Tagger, M., Muno, M., Morris, M., \& Cowley, S. 2005, ApJ, 631, L53

\bibitem[Belmont \& Tagger(2006)]{be06} Belmont, R. \& Tagger, M. 2006, A\&A, 452, 15

\bibitem[Benford(1988)]{b88} Benford, G. 1988, ApJ, 333, 735

\bibitem[Binney et al.(1991)]{bi91} Binney, J., Gerhard, O. E., Stark, A. A., Bally, J., \& Uchida, K. I. 1991, MNRAS, 252, 210

\bibitem[Blair et al.(1999)]{bl99} Blair, W. P., Sankrit, R., Raymond, J. C., \& Long, K. S. 1999, AJ, 118, 942

\bibitem[Bland-Hawthorn \& Cohen(2003)]{b03} Bland-Hawthorn, J \& Cohen, M. 2003, ApJ, 582, 246

\bibitem[Bloemen(1987)]{bl87} Bloemen, J. B. G. M. 1987, ApJ, 322, 694

\bibitem[Blommaert et al.(1998)]{b98} Blommaert, J. A. D. L., van der Veen, W. E. C. J., van Langevelde, H. J., Habing, H. J., \& Sjouwerman, L. O. 1998, A\&A, 329, 991

\bibitem[Boldyrev \& Yusef-Zadeh(2006)]{b06} Boldyrev, S. \& Yusef-Zadeh, F. 2006, ApJ, 637L, 101

\bibitem[Bower et al.(2004)]{bo04} Bower, G. C., Falcke, H., Herrnstein, R. M., Zhao, J.-H., Goss, W. M., Backer, D. C. 2004, Science, 304, 704

\bibitem[Bower et al.(2005)]{bo05} Bower, G. C., Falcke, H., Wright, M. C., \& Backer, D. C. 2005, ApJ, 618, L29

\bibitem[Blundell \& Rawlings(2000)]{b00} Blundell, K. M. \& Rawlings, S. 2000, AJ, 119, 1111

\bibitem[Breitschwerdt et al.(1991)]{b91} Breitschwerdt, D., Voelk, H. J., \& McKenzie, J. F. 1991, A\&A, 245, 79

\bibitem[Bridle \& Schwab(1999)]{b99} Bridle, A. H. \& Schwab, F. S. 1999, Synthesis Imaging in Radio Astronomy II, ASP, 180, 371

\bibitem[Brocklehurst(1970)]{b70} Brocklehurst, M. 1970, MNRAS, 148, 417

\bibitem[Brocklehurst \& Seaton(1972)]{b72} Brocklehurst, M. \& Seaton, M. J. 1972, MNRAS, 157, 179

\bibitem[Broderick \& Narayan(2006)]{br06} Broderick, A. E. \& Narayan, R. 2006, ApJ, 638L, 21

\bibitem[Brogan \& Goss(2003)]{b03a} Brogan, C. \& Goss, W. M. 2003, AJ, 125, 272

\bibitem[Brogan et al.(2003)]{b03b} Brogan, C. L., Nord, M., Kassim, N., Lazio, J., \& Anantharamaiah, K. 2003, ANS, 324, 17

\bibitem[Brown \& Johnston(1983)]{b83} Brown, R. L. \& Johnston, K. J. 1983, ApJ, 268, L85

\bibitem[Burn(1966)]{b66} Burn, B. J., 1966, MNRAS, 133, 67

\bibitem[Carigi et al.(2005)]{c05} Carigi, L., Peimbert, M., Esteban, C., Garc\'ia-Rojas, J. 2005, ApJ, 623, 213

\bibitem[Cecil et al.(1990)]{ce90} Cecil, G., Bland, J., \& Tully, R. B. 1990, ApJ, 355, 70

\bibitem[Cersosimo \& Magnani(1990)]{c90} Cersosimo, J. C. \& Magnani, L. 1990, A\&A, 239, 287

\bibitem[Chevalier(1992)]{c92} Chevalier, R. A. 1992, ApJ, 397, L39

\bibitem[Chevalier \& Clegg(1985)]{c85} Chevalier, R. A. \& Clegg, A. W. 1985, Nature, 317, 44

\bibitem[Christopher et al.(2005)]{ch05} Christopher, M. H., Scoville, N. Z., Stolovy, S. R., \& Yun, Min S. 2005, ApJ, 622, 346

\bibitem[Chu \& Kennicutt(1994)]{c94} Chu, Y.-H. \& Kennicutt, R. C., Jr. 1994, ApJ, 425, 720

\bibitem[Churches et al.(2001)]{c01} Churches, D. K., Nelson, A. H., \& Edmunds, M. G. 2001, MNRAS, 327, 610

\bibitem[Chuss et al.(2003)]{c03} Chuss, D. T., Davidson, J. A., Dotson, J. L., Dowell, C. D., Hildebrand, R. H., Novak, G., \& Vaillancourt, J. E. 2003, ApJ, 599, 1116

\bibitem[Clark \& Caswell(1976)]{c76} Clark, D. H. \& Caswell, J. L. 1976, MNRAS, 174, 267

\bibitem[Clark et al.(2005)]{cl05} Clark, J. S., Negueruela, I., Crowther, P. A., \& Goodwin, S. P. 2005, A\&A, 434, 949

\bibitem[Condon et al.(1998)]{c98} Condon, J. J. et al.\ 1998, AJ, 115, 1693

\bibitem[Cordes \& Lazio(2004)]{c04} Cordes, J. M. \& Lazio, T. J. W. 2004, astro-ph/0207156

\bibitem[Cordes \& Rickett(1998)]{co98} Cordes, J. M. \& Rickett, B. J. 1998, ApJ, 507, 846

\bibitem[Cotera et al.(2005)]{co05} Cotera, A. S., Colgan, S. W. J., Simpson, J. P., \& Rubin, R. H. 2005, ApJ, 622, 333

\bibitem[Cotera et al.(1996)]{c96} Cotera, A. S., Erickson, E. F., Colgan, S. W. J., Simpson, J. P., Allen, D. A., \& Burton, M. G. 1996, ApJ, 461, 750

\bibitem[Cotera et al.(1999)]{ca99} Cotera, A., et al. 1999, ApJ, 510, 747

\bibitem[Cotera et al.(2007)]{c07} Cotera, A., et al. 2007, in preparation

\bibitem[Cotton(1999)]{c99} Cotton, W. D. 1999, Synthesis Imaging in Radio Astronomy II, ASP, 180, 120

\bibitem[Cox \& Laureijs(1989)]{c89} Cox, P. \& Laureijs, R. 1989, IAUS, 137, 121

\bibitem[Dahlburg et al.(2002)]{d02} Dahlburg, R. B., Einaudi, G., LaRosa, T. N., \& Shore, S. N. 2002, ApJ, 568, 220

\bibitem[Dame et al.(2001)]{d01} Dame, T. M., Hartmann, D., \& Thaddeus, P. 2001, ApJ, 547, 792

\bibitem[Davies et al.(1976)]{d76} Davies, R. D., Walsh, D., \& Booth, R. S. 1976, MNRAS, 177, 319

\bibitem[De Pree et al.(2005)]{d05} De Pree, C. G., Wilner, D. J., Deblasio, J., Mercer, A. J., \& Davis, L. E. 2005, ApJ, 624L, 101

\bibitem[Downes \& Maxwell(1966)]{d66} Downes, D. \& Maxwell, A. 1966, ApJ, 146, 653

\bibitem[Dravskikh \& Dravskikh(1964)]{d64} Dravskikh, Z. V. \& Dravskikh, A. F. 1964, Astron. Tsirk., 158, 2

\bibitem[Duncan et al.(1995)]{d95} Duncan, A. R., Stewart, R. T., Haynes, R. F., \& Jones, K. L. 1995, MNRAS, 277, 36

\bibitem[Dunn \& Fabian(2004)]{d04} Dunn, R. J. H., \& Fabian, A. C. 2004, MNRAS, 355, 862

\bibitem[Dupree(1969)]{d69} Dupree, A. K. 1969, ApJS, 18, 221

\bibitem[Dupree(1972)]{d72} Dupree, A. K. 1972, ApJ, 173, 293

\bibitem[Dupree \& Goldberg(1970)]{d70} Depree, C. G. \& Goldberg, L. 1970, ARA\&A, 8, 231

\bibitem[Eckart et al.(2006)]{e06} Eckart, A. et al. 2006, A\&A, 450, 535

\bibitem[Ekers et al.(1983)]{e83} Ekers, R. D., van Gorkom, J. H., Schwarz, U. J., \& Goss, W. M. 1983, A\&A, 122, 143

\bibitem[Elmouttie et al.(1998)]{e98} Elmouttie, M., Haynes, R. F., Jones, K. L., Sadler, E. M., \& Ehle, M. 1998, MNRAS, 297, 1202

\bibitem[Falcke et al.(2004)]{fa04} Falcke, H., K\"ording, E., \& Markoff, S. 2004, A\&A, 414, 895

\bibitem[Falcke \& Markoff(2000)]{fa00} Falcke, H. \& Markoff, S. 2000, A\&A, 362, 113

\bibitem[Fanaroff \& Riley(1974)]{f74} Fanaroff, B. L. \& Riley, J. M. 1974, MNRAS, 167, 31

\bibitem[Faraday(1844)]{f44} Faraday, M. 1844, Experimental Researches in Electricity (London: R. Taylor), reprinted 1942 (New York: Dover)

\bibitem[Fender \& Kuulkers(2001)]{f01} Fender, R. P. \& Kuulkers, E. 2001, MNRAS, 324, 923

\bibitem[Ferrarese et al.(2001)]{fe01} Ferrarese, L., Pogge, R. W., Peterson, B., M., Merritt, D., Wandel, A., \& Joseph, C. L. 2001, ApJ, 555L, 79

\bibitem[Figer et al.(2006)]{f06} Figer, D. F. et al. 2006, ApJ, accepted, astro-ph/0602146

\bibitem[Figer et al.(2004)]{f04} Figer, D. F., Rich, R. M., Kim, S. S., Morris, M., \& Serabyn, E. 2004, ApJ, 601, 319

\bibitem[Figer et al.(1999)]{f99} Figer, D. F., McLean, I. S. \& Morris, M. 1999, ApJ, 514, 202

\bibitem[Fletcher \& Shukurov(2006)]{fl06} Fletcher, A. \& Shukurov, A. 2006, MNRAS, 371, L21

\bibitem[Fragile \& Mathews(2000)]{f00} Fragile, P. C. \& Mathews, J. 2000, ApJ, 542, 328

\bibitem[Frail et al.(1996)]{f96} Frail, D. A., Goss, W. M., Reynoso, E. M., Giacani, E. B., Green, A. J. \& Otrupcek, R. 1996, AJ, 111, 1651

\bibitem[Gallo et al.(2005)]{ga05} Gallo, E. 2005, Nature, 436, 819

\bibitem[Gaensler et al.(2001)]{g01} Gaensler, B. M., Dickey, J. M., McClure-Griffiths, N. M., Green, A. J., Wieringa, M. H., \& Haynes, R. F. 2001, ApJ, 549, 959

\bibitem[Gaensler et al.(2003)]{g03} Gaensler, B., Fogel, J. K. J., Slane, P. O., Miller, J. M., Wijnands, R., Eikenberry, S. S., \& Lewin, W. H. G. 2003, ApJ, 594, L35

\bibitem[Gaume et al.(1995)]{ga95} Gaume, R. A., Claussen, M. J. , De Pree, C. G., Goss. W. M. \& Mehringer, D. M. 1995, ApJ, 449, 663

\bibitem[Gehrels(1986)]{g86} Gehrels, N. 1986, ApJ, 303, 336

\bibitem[Gelfand et al.(2004)]{g04} Gelfand, J. D., Lazio, T. J. W., \& Gaensler, B. M. 2004, ApJS, 155, 89

\bibitem[Gelfand et al.(2005)]{ge05} Gelfand, J. D., Lazio, T. J. W., \& Gaensler, B. M. 2005, ApJS, 159, 242

\bibitem[Genzel \& Townes(1987)]{g87} Genzel, R. \& Townes, C. H. 1987, ARA\&A, 25, 377

\bibitem[Ghez et al.(2005)]{g05} Ghez, A., et al. 2005, ApJ, 620, 744

\bibitem[Giveon et al.(2005a)]{g05a} Giveon, U., Becker, R. H.,  Helfand, D. J., \& White, R. L. 2005, AJ, 129, 348

\bibitem[Giveon et al.(2005b)]{g05b} Giveon, U., Becker, R. H.,  Helfand, D. J., \& White, R. L. 2005, AJ, 130, 156

\bibitem[Goetz \& Koeppen(1992)]{g92} Goetz, M. \& Koeppen, J. 1992, A\&A, 262, 455

\bibitem[Gordon(1974)]{g74} Gordon, M. A. 1974, IAUS, 60, 477

\bibitem[Goss et al.(2003)]{go03} Goss, W. M., Brown, Robert L., \& Lo, K. Y. 2003, ANS, 324, 497

\bibitem[Goss \& Shaver(1970)]{g70} Goss, W. M. \& Shaver, P. A. 1970, AuJPA, 14, 1

\bibitem[Gaustad et al.(2001)]{ga01} Gaustad, J. E., McCullough, P. R., Rosing, W. and Van Buren, D. 2001, PASP, 113, 1326

\bibitem[Gray(1994)]{g94} Gray, A. D. 1994, MNRAS, 270, 835

\bibitem[Gray et al.(1993)]{g93} Gray, A. D., et al. 1993, MNRAS, 264, 678

\bibitem[Gray et al.(1995)]{g95} Gray, A.D., Nicholls, J., Ekers, R. D., \& Cram, L. E. 1995, ApJ, 448, 164

\bibitem[Green(2004)]{gr04} Green, D. A., 2004, Bulletin of the Astronomical Society of India, 32, 335

\bibitem[G\"urkan \& Rasio(2005)]{gu05} G\"urkan, M. A. \& Rasio, F. A. 2005, ApJ, 628, 236

\bibitem[Han et al.(2006)]{h06} Han, J. L., Manchester, R. N., Lyne, A. G.,Qiao, G. J.,van Straten, W. 2006, astro-ph/0601357

\bibitem[Han et al.(1999)]{h99} Han, J. L., Manchester, R. N., \& Qiao, G. J. 1999, MNRAS, 306, 371

\bibitem[Handa et al.(1987)]{ha87} Handa, T., Sofue, Y., Nakai, N., Hirabayashi, H., \& Inoue, M. 1987, PASJ, 39, 709

\bibitem[Haverkorn et al.(2000)]{h00} Haverkorn, M., Katgert, P., \& de Bruyn, A. G. 2000, A\&A, 356, L13

\bibitem[Haverkorn et al.(2004)]{h04} Haverkorn, M., Katgert, P., \& de Bruyn, A. G. 2004, A\&A, 427, 549

\bibitem[Haynes et al.(1992)]{h92} Haynes, R. F., Stewart, R. T., Gray, A. D., Reich, W., Reich ,P., \& Mebold, U. 1992, A\&A, 264, 500

\bibitem[Heckman et al.(1990)]{h90} Heckman, T. M., Armus, L., \& Miley, G. K. 1990, ApJS, 74, 833

\bibitem[Heiles et al.(1996)]{h96} Heiles, C., Reach, W. T., \& Koo, B.-C. 1996, ApJ, 466, 191

\bibitem[Helfand \& Becker(1987)]{h87} Helfand, D. J. \& Becker, R. H. 1987, ApJ, 314, 203

\bibitem[Heyvaerts et al.(1988)]{h88} Heyvaerts, J., Norman, C., \& Pudritz, R. E. 1988, ApJ, 330, 718

\bibitem[Hyman et al.(2002)]{h02} Hyman, S. D., Lazio, T. J. W., Kassim, N. E., \& Bartleson, A. L. 2002, AJ, 123, 1497

\bibitem[Hyman et al.(2005)]{h05} Hyman, S. D., Lazio, T. J. W., Kassim, N. E., Ray, P. S., Markwardt, C. B., \& Yusef-Zadeh, F. 2005, Nature, 434, 50

\bibitem[Isaacman(1981)]{i81} Isaacman, R. 1981, A\&AS, 43, 405

\bibitem[Jaffe \& Perola(1973)]{j73} Jaffe, W. J. \& Perola, G. C. 1973, A\&A, 26, 423

\bibitem[Jogee et al.(2005)]{j05} Jogee, S., Scoville, N., \& Kenney, J. D. P. 2005, ApJ, 630, 837

\bibitem[Kaplan et al.(2000)]{k00} Kaplan, D. L., Cordes, J. M., \& Condon, J. J. 2000, ApJS, 126, 37

\bibitem[Kardashev(1959)]{k59} Kardashev, N. S. 1959, Soviet Astr., 3, 813

\bibitem[Kassim \& Frail(1996)]{ka96} Kassim, N. E. \& Frail, D. A. 1996, MNRAS, 283, L51

\bibitem[Kim et al.(2004)]{k04} Kim, S. S., Figer, D. F., \& Morris, M. 2004, ApJ, 607L, 123

\bibitem[Kinney et al.(2000)]{ki00} Kinney, A. L., Schmitt, H. R., Clarke, C. J., Pringle, J. E., Ulvestad, J. S., \& Antonucci, R. R. J. 2000, ApJ, 537, 152

\bibitem[Koyama et al.(1996)]{k96} Koyama, K., Maeda, Y., Sonobe, T., Takeshima, T., Tanaka, Y., \& Yamauchi, S. 1996, PASJ, 48, 249

\bibitem[Kruegel et al.(1983)]{k83} Kruegel, E., Tutukov, A., \& Loose, H. 1983, A\&A,124, 89

\bibitem[Lang et al.(1999a)]{la99} Lang, C. C., Anantharamaiah, K.R., Kassim, N.E., \& Lazio, T. J. W. 1999, ApJ, 521L, 41

\bibitem[Lang et al.(2002)]{l02} Lang, C. C., Goss, W. M., \& Morris, M. 2002, AJ, 124, 2677

\bibitem[Lang et al.(1997)]{l97} Lang, C. C., Goss, W. M., \& Wood, D. O. S. 1997, ApJ, 474, 275

\bibitem[Lang et al.(1999b)]{l99} Lang, C. C., Morris, M., Echevarria, L. 1999, ApJ, 526, 727

\bibitem[Lang(1971)]{l71} Lang, K. R. 1971, ApJ, 164, 249

\bibitem[Lang(1974)]{l74} Lang, K. R. 1974, Astrophysical Formulae, Springer-Verlag, Berlin

\bibitem[Lang \& Willson(1978)]{l78} Lang, K. R. \& Willson, R. F. 1978, ApJ, 219, 474

\bibitem[LaRosa et al.(2005)]{la05} LaRosa, T. N., Brogan, C. L., Shore, S. N., Lazio, T. J., Kassim, N. E., \& Nord, M. E.  2005, ApJ, 626, L23

\bibitem[LaRosa et al.(2000)]{l00} LaRosa, T. N., Kassim, N. E., Lazio, T. J. W., \& Hyman, S. D. 2000, AJ, 119, 207

\bibitem[LaRosa et al.(2001)]{l01} LaRosa, T. N., Lazio, T. J. W., \& Kassim, N. E.2001, ApJ, 563, 163

\bibitem[LaRosa et al.(2004)]{l04} LaRosa, T. N., Nord, M. E., J., T., Lazio, W., \& Kassim, N. E.  2004, ApJ, 607, 302

\bibitem[Launhardt et al.(2002)]{la02} Launhardt, R., Zylka, R., \& Mezger, P. G. 2002, A\&A, 384, 112

\bibitem[Lasenby et al.(1989)]{l89} Lasenby, J., Lasenby, A. N., \& Yusef-Zadeh, F. 1989, ApJ, 343, 177

\bibitem[Lazendic et al.(2002)]{laz02} Lazendic, J. S., Wardle, M., Burton, M. G., Yusef-Zadeh, F., Whiteoak, J. B., Green, A. J., \& Ashley, M. C. B.  2002, MNRAS, 331, 537

\bibitem[Lazio \& Cordes(1998a)]{l98} Lazio, T. J. W. \& Cordes, J. M. 1998, ApJS, 118, 201

\bibitem[Lazio \& Cordes(1998b)]{l98b} Lazio, T. J. W. \& Cordes, J. M. 1998, ApJ, 505, 715

\bibitem[Leahy(1989)]{le89} Leahy, D. A. 1989, A\&A, 216, 193

\bibitem[Lehnert et al.(1999)]{le99} Lehnert, M. D., Heckman, T. M., \& Weaver, K. A. 1999, ApJ, 523, 575

\bibitem[Lerche \& Schlickeiser(1982)]{l82} Lerche, I. \& Schlickeiser, R. 1982, A\&A, 107, 148

\bibitem[Lilley \& Palmer(1968)]{l68} Lilley, A. E. \& Palmer, P. 1968, ApJS, 16, 143

\bibitem[Lindqvist et al.(1992)]{li92} Lindqvist, M., Habing, H. J., \& Winnberg, A. 1992, A\&A, 259, 118

\bibitem[Lis \& Carlstrom(1994)]{l94} Lis, D. C. \& Carlstrom, J. E. 1994, ApJ, 424, 189

\bibitem[Lis \& Goldsmith(1989)]{li89} Lis, D. C. \& Goldsmith, P. F. 1989, ApJ, 337, 704

\bibitem[Liszt(1992)]{l92} Liszt, H. S. 1992, ApJS, 82, 495

\bibitem[Liszt(2006)]{l06} Liszt, H. S. 2006, A\&A, 447, 533

\bibitem[Liszt \& Spiker(1995)]{l95} Liszt, H. S. \& Spiker, R. W. 1995, ApJS, 98, 259

\bibitem[Little(1974)]{li74} Little, A. G. 1974, IAUS, 60, 491

\bibitem[Liu \& Melia(2002)]{li02} Liu, S. \& Melia, F. 2002, ApJ, 566L, 77

\bibitem[Lo et al.(1975)]{l75} Lo, K. Y., Schilizzi, R. T., Cohen, M. H., \& Ross, H. N. 1975, ApJ, 202L, 63

\bibitem[Lockman \& Gordon(1973)]{l73} Lockman, F. J. \& Gordon, M. A. 1973, ApJ, 182, 25

\bibitem[Lorimer et al.(1995)]{lo95} Lorimer, D. R., Yates, J. A., Lyne, A. G., \& Gould, D. M. 1995, MNRAS, 273, 411

\bibitem[Mac Low \& McCray(1988)]{m88} Mac Low, M-M. \& McCray, R. 1988, ApJ, 324, 776

\bibitem[Maeda et al.(2002)]{m02} Maeda, Y. 2002, ApJ, 570, 671

\bibitem[Manchester(1987)]{m87} Manchester R.N. 1987, A\&A, 171, 205

\bibitem[Manchester et al.(2005)]{ma05} Manchester, R. N., Hobbs, G. B., Teoh, A. \& Hobbs, M. 2005, AJ, 129, 1993 (See also \url{http://www.atnf.csiro.au/research/pulsar/psrcat})

\bibitem[Markoff(2005)]{mar05} Markoff, S. 2005, ApJ, 618L, 103

\bibitem[Martin(2005)]{m05} Martin, C. L. 2005, 621, 227

\bibitem[Martin et al.(2004)]{ma04} Martin, C. L., Walsh, W. M., Xiao, K., Lane, A. P., Walker, C. K., \& Stark, A. A. 2004, ApJS, 150, 239

\bibitem[Martins \& Viegas(2000)]{m00} Martins, L. P. \& Viegas, S. M. M. 2000, A\&A, 361, 1121

\bibitem[Mathis(1985)]{m85} Mathis, J. S. 1985, ApJ, 291, 247

\bibitem[Maugherhan et al.(2005)]{mg05}	Mauerhan, J. C., Morris, M., Walter, F., \& Baganoff, F. K. 2005, ApJ, 623L, 25

\bibitem[Mehringer et al.(1993)]{m93} Mehringer, D. M., Palmer, P., Goss. W. M. \& Yusef-Zadeh, F. 1993, ApJ, 412, 684

\bibitem[Mehringer et al.(1992)]{m92} Mehringer, D. M., Yusef-Zadeh, F., Palmer, P., \& Goss, W. M. 1992, ApJ, 401, 168

\bibitem[Melia \& Falcke(2001)]{m01} Melia, F. \& Falcke, H. 2001, ARA\&A, 39, 309

\bibitem[Melia et al.(1998)]{m98} Melia, F., Yusef-Zadeh, F., \& Fatuzzo, M. 1998, ApJ, 508, 676

\bibitem[Menzel(1969)]{m69} Menzel, D. H. 1969, ApJS, 18, 221

\bibitem[Mezger \& Henderson(1967)]{m67} Mezger, P. G. \& Henderson, A. P. 1967, ApJ, 147, 471

\bibitem[Mezger et al.(1989)]{m89} Mezger, P. G., Zylka, R., Salter, C. J., Wink, J. E., Chini., R., Kreysa, E., \& Tuffs, R. 1989, A\&A, 209, 337

\bibitem[Moffat(1975)]{m75} Moffat, A. T. 1975, in Galaxies and the Universe: Stars and Stellar Systems, Vol. 9, ed. A. Sandage, M. Sandage, \& J. Kristian (Chicago: Univ. Chicago Press), 211

\bibitem[Morris \& Serabyn(1996)]{m96} Morris, M. \& Serabyn, E. 1996, ARA\&A, 34, 645

\bibitem[Morris et al.(2006)]{m06} Morris, M., Uchida, K., \& Do, T. 2006, Nature, 440, 308

\bibitem[Muno et al.(2004)]{m04} Muno, M. P. et al. 2004, ApJ, 613, 326

\bibitem[Muno et al.(2005)]{mu05} Muno, M. P., Pfahl, E., Baganoff, F. K., Brandt, W. N., Ghez, A., Lu, J., \& Morris, M. R. 2005, ApJ, 622, L113

\bibitem[Nagata et al.(1990)]{n90} Nagata, T., Woodward, C. E., Shure, M., Pipher, J. L., \& Okuda, H. 1990, ApJ, 351, 83

\bibitem[Nord et al.(2004)]{n04} Nord, M. E., Lazio, T. J. W., Kassim, N. E., Hyman, S. D., LaRosa, T. N., Brogan, C. L., \& Duric, N. 2004, AJ, 128, 1646 (erratum 131, 1886, [2006])

\bibitem[Novak et al.(2003)]{n03} Novak, G., et al. 2003, ApJ, 583L, 83

\bibitem[Nummelin et al.(2000)]{n00} Nummelin, A. et al. 2000, ApJS, 128, 213

\bibitem[O'Dea(1998)]{o98} O'Dea, C. P. 1998, PASP, 110, 493

\bibitem[Oka et al.(2005)]{o05} Oka, T., Geballe, T. R., Goto, M., Usuda, T., \& McCall, B. J. 2005, ApJ, 632, 882

\bibitem[Pacholczyk(1970)]{p70} Pacholczyk, A. G. 1970, Radio Astrophysics, Freeman and Co., San Francisco

\bibitem[Panagia \& Walmsley(1978)]{p78} Panagia, N. \& Walmsley, C. M. 1978, A\&A, 70, 411

\bibitem[Pauls \& Mezger(1975)]{p75} Pauls, T. \& Mezger, P. G. 1975, A\&A, 182, 25

\bibitem[Peck et al.(1997)]{p97} Peck, A. B., et al. 1997, ApJ, 486, 329

\bibitem[Pedlar et al.(1989)]{p89} Pedlar, A., Anantharamaiah, K. R., Ekers, R. D., Goss, W. M., van Gorkom, J. H., Schwarz, U. J., \& Zhao, J-H. 1989, ApJ, 342, 769

\bibitem[Peeters et al.(2004)]{p04} Peeters, E., Spoon, H. W. W., \& Tielens, A. G. G. M. 2004, ApJ, 613, 986

\bibitem[Perley et al.(1984)]{p84} Perley, R. A., Dreher, J. W., \& Cowan, J. J. 1984, ApJ, 285L, 35

\bibitem[Platania et al.(1998)]{p98} Platania, et al. 1998, ApJ, 505, 473

\bibitem[Pohl et al.(1992)]{pr92} Pohl, M., Reich, W., \& Schlickeiser, R. 1992, A\&A, 262, 441

\bibitem[Pohl \& Schlickeiser(1992)]{p92} Pohl, M. \& Schlickeiser, R. 1992, A\&A, 263, 37

\bibitem[Portegies Zwart et al.(2003)]{p03} Portegies Zwart, S. F., McMillan, S. L. W., \& Gerhard, O. 2003, ApJ, 593, 352

\bibitem[Price et al.(2001)]{p01} Price, S. D., Egan, M. P., Carey, S. J., Mizuno, D. R., \& Kuchar, T. A. 2001, AJ, 121, 2819

\bibitem[Reich(2003)]{re03} Reich, W. 2003, A\&A, 401, 1023

\bibitem[Reich \& F\"urst(1984)]{r84} Reich, W. \& F\"urst, E. 1984, A\&AS, 57, 165

\bibitem[Reich et al.(1987)]{r87} Reich, W., Sofue, Y., \& Fuerst, E. 1987, PASJ, 39, 573

\bibitem[Reich \& Reich(1988a)]{r88a} Reich, P. \& Reich, W. 1988, A\&AS, 74, 7

\bibitem[Reich \& Reich(1988b)]{r88b} Reich, P. \& Reich, W. 1988, A\&A, 196, 211

\bibitem[Reich et al.(1990)]{r90} Reich, W., Reich, P., \& F\"urst, E. 1990, A\&AS, 83, 539

\bibitem[Reid(1993)]{r93} Reid, M. J. 1993, ARA\&A, 31, 345

\bibitem[Revnivtsev et al.(2004)]{r04} Revnivtsev, M. G. et al. 2004, A\&A, 425L, 49

\bibitem[Ribas et al.(2005)]{ri05} Ribas, I., Jordi, C., Vilardell, F., Fitzpatrick, E. L., Hilditch, R. W., \& Guinan, E. F. 2005, ApJ, 635L, 37

\bibitem[Roberge et al.(1995)]{r95} Roberge, W. G., Hanany, S., \& Messinger, D. W. 1995, ApJ, 453, 238

\bibitem[Roberts \& Goss(1993)]{ro93} Roberts, D. A. \& Goss, W. M. 1993, ApJS, 86, 133

\bibitem[Roberts et al.(1996)]{r96} Roberts, D. A., Yusef-Zadeh, F., \& Goss, W. M. 1996, ApJ, 459, 627

\bibitem[Rodr\'iguez-Fern\'andez \& Mart\'in-Pintado(2005)]{ro05} Rodr\'iguez-Fern\'andez, N. J. \& Mart\'in-Pintado, J. 2005, A\&A, 429, 923

\bibitem[Rodr\'iguez-Fern\'andez et al.(2001)]{r01} Rodr\'iguez-Fern\'andez, N. J., Mart\'in-Pintado, J., \& de Vicente, P. 2001, A\&A, 377, 631

\bibitem[Roelfsema \& Goss(1992)]{r92} Roelfsema, P. R. \& Goss, W. M. 1992, A\&A Rev., 4, 161

\bibitem[Roelfsema et al.(1989)]{r89} Roelfsema, P. R., Goss, W. M., \& Geballe, T. R. 1989, A\&A, 222, 247

\bibitem[Rohlfs \& Braunsfurth(1982)]{r82} Rohlfs, K. \& Braunsfurth, E. 1982, A\&A, 113, 237

\bibitem[Roy(2003)]{r03} Roy, S. 2003, A\&A, 403, 917

\bibitem[Roy et al.(2005)]{r05} Roy, S., Rao, A. P., \& Subrahmanyan, R. 2005, MNRAS, 360, 1305

\bibitem[Russeil(2003)]{ru03} Russeil, D. 2003, A\&A, 397, 133

\bibitem[Rybicki \& Lightman(1979)]{r79} Rybicki, G. B. \& Lightman, A. P. 1979, Radiative Processes in Astrophysics, John Wiley \& Sons, Inc., New York

\bibitem[Salem \& Brocklehurst(1979)]{s79} Salem, M. \& Brocklehurst, M. 1979, ApJS, 39, 633

\bibitem[Sato et al.(2000)]{s00} Sato, F. Hasegawa, T., Whiteoak, J. B., \& Miyawaki, R. 2000, ApJ, 535, 857

\bibitem[Sawada et al.(2004)]{s04} Sawada, T., Hasegawa, T., Handa, T., \& Cohen, R. J. 2004, MNRAS, 349, 1167

\bibitem[Scheffler \& Els\"asser(1988)]{s88} Scheffler, H., \& Els\"asser, H. 1988, in Physics of the Galaxy and Interstellar Matter, Springer-Verlag, pg. 271

\bibitem[Sch\"odel et al.(2003)]{sc03} Sch\"odel, R., Ott, T., Genzel, R., Eckart, A., Mouawad, N., \& Alexander, T. 2003, ApJ, 596, 1015

\bibitem[Schmidt(1978)]{s78} Schmidt, J. 1978, Ph.D. thesis, Univ. of Bonn

\bibitem[Schmitt et al.(2003)]{sch03} Schmitt, H. R., Donley, J. L., Antonucci, R. R. J., Hutchings, J. B., \& Kinney, A. L. 2003, ApJS, 148, 327

\bibitem[Seaquist \& Clark(2001)]{s01} Seaquist, E. R. \& Clark, J. 2001, ApJ, 552, 133

\bibitem[Serabyn \& Morris(1994)]{s94} Serabyn, E. \& Morris, M. 1994, ApJ, 424, L91

\bibitem[Shaver(1980)]{s80} Shaver, P. A. 1980, A\&A, 91, 279

\bibitem[Shaver et al.(1983)]{s83} Shaver, P. A., McGee, R. X., Newton, L. M., Danks, A. C., \& Pottasch, S. R. 1983, MNRAS, 204, 53

\bibitem[Shibata \& Uchida(1987)]{su87} Shibata, K. \& Uchida, Y. 1987, PASJ, 39, 559

\bibitem[Shopbell \& Bland-Hawthorn(1998)]{s98} Shopbell, P. L. \& Bland-Hawthorn, J. 1998, ApJ, 493, 129

\bibitem[Shore \& LaRosa(1999)]{s99} Shore, S. N. \&  LaRosa, T. N. 1999, ApJ, 521, 587

\bibitem[Shu et al.(1987)]{sh87} Shu, F. H., Adams, F. C., \& Lizano, S. 1987, ARA\&A, 25, 23

\bibitem[Shull(1987)]{s87} Shull, J. M. 1987 in Interstellar Processes, D. J. Hollenbach, H. A. Thronson, eds., pg. 225

\bibitem[Simard-Normandin \& Kronberg(1980)]{si80} Simard-Normandin, M. \& Kronberg, P. P. 1980, ApJ, 242, 74

\bibitem[Smith et al.(2002)]{sm02} Smith, L. J., Norris, R. P. F., \& Crowther, P. A. 2002, MNRAS, 337 ,1309

\bibitem[Sofue(1985)]{s85} Sofue, Y. 1985, PASJ, 37, 697

\bibitem[Sofue(1995)]{s95} Sofue, Y. 1995, PASJ, 47, 527

\bibitem[Sofue(1996)]{s96} ------ 1996, ApJ, 459, L69

\bibitem[Sofue(2003)]{s03} ------ 2003, PASJ, 55, 445

\bibitem[Sofue \& Handa(1984)]{s84} Sofue, Y. \& Handa, T. 1984, Nature, 310, 568

\bibitem[Sofue et al.(1992)]{so92} Sofue, Y., Murata, Y., \& Reich, W. 1992, PASJ, 44, 367

\bibitem[Sokoloff et al.(1998)]{so98} Sokoloff, D. D., et al. 1998, MNRAS, 299, 189

\bibitem[Sorochenko \& Borozich(1964)]{s64} Sorochenko, R. L. \& Borozich, E. V. 1964, Rep. of the Sov. Acad. of Science, 162, 3, 603

\bibitem[Spergel \& Blitz(1992)]{s92} Spergel, D. N. \& Blitz, L. 1992, Nature, 357, 665

\bibitem[Stanimirovi\'c(2002)]{s02} Stanimirovi\'c, S. 2002, Short-Spacings Correction from the Single-Dish Perspective, ASPC, 278, 375, eds. Stanimirovi\'c et al.

\bibitem[Stark et al.(1992)]{st92} Stark, A. A., Gammie, C. F., Wilson, R. W., Bally, J., Linke, R. A., Heiles, C., \& Hurwitz, M. 1992, ApJS, 79, 77

\bibitem[Stark et al.(2004)]{st04} Stark, A. A., Martin, C. L., Walsh, W. M., Xiao, K., Lane, A. P., Walker, C. K. 2004, ApJ, 614L, 41

\bibitem[Steffen et al.(1997)]{s97} Steffen, W., Gomez, J. L., Raga, A. C., \& Williams, R. J. R. 1997, ApJ, 491L, 73

\bibitem[Stevens \& Hartwell(2003)]{st03} Stevens, I. R. \& Hartwell, J. M. 2003, MNRAS, 339, 280

\bibitem[Stolovy et al.(2007)]{s07} Stolovy, S., et al. 2007, in preparation

\bibitem[Suchkov et al.(1994)]{su94} Suchkov, A. A., Balsara, D. S., Heckman, T. M., \& Leitherner, C. 1994, ApJ, 430, 511

\bibitem[Sunyaev \& Churazov(1998)]{su98} Sunyaev, R. \& Churazov, E. 1998, MNRAS, 297, 1279

\bibitem[Taylor \& Cordes(1993)]{t93} Taylor, J. H. \& Cordes, J. M. 1993, ApJ, 411, 674

\bibitem[Taylor et al.(1992)]{t92} Taylor, D., Dyson, J. E., \& Axon, D. J. 1992, MNRAS, 255, 351

\bibitem[Thurow \& Wilcots(2005)]{t05} Thurow, J. C. \& Wilcots, E. M. 2005, AJ, 129, 745

\bibitem[Tsuboi et al.(1995)]{t95} Tsuboi, M., Kawabata, T., Kasuga, T., Handa, T., Kato, T. 1995, PASJ, 47, 829

\bibitem[Tsuboi et al.(1986)]{t86} Tsuboi, M., et al. 1986, AJ, 92, 818

\bibitem[Uchida et al.(1992)]{u92} Uchida, K. I., Morris, M., Bally, J., Pound, M., \& Yusef-Zadeh, F. 1992, ApJ, 398, 128

\bibitem[Uchida et al.(1990)]{u90} Uchida, K., Morris, M., \& Serabyn, E. 1990, ApJ, 351, 443

\bibitem[Uchida et al.(1994)]{u94} Uchida, K. I., et al.\ 1994, ApJ, 421, 505

\bibitem[Uchida et al.(1985)]{u85} Uchida, Y., Shibata, K., \& Sofue, Y. 1985, Nature, 317, 699

\bibitem[Uyaniker et al.(2003)]{u03} Uyaniker, B., Landecker, T. L., Gray, A. D., \& Kothes, R. 2003, ApJ, 585, 785

\bibitem[van Langevelde et al.(1992)]{v92} van Langevelde, H. J., Frail, D. A., Cordes, J. M., \& Diamond, P. J. 1992, ApJ, 396, 686

\bibitem[Veilleux et al.(2005)]{v05} Veilleux, S., Cecil, G., \& Bland-Hawthorn, J. 2005, ARA\&A, 43, 769

\bibitem[Veilleux et al.(1994)]{v94} Veilleux, S., Cecil, G., Bland-Hawthorn, J., Tully, R. B., Filippenko, A. V., \& Sargent, W. L. W. 1994, ApJ, 433, 48

\bibitem[Walter et al.(1998)]{w98} Walter, F., Kerp, J., Duric, N., Brinks, E., \& Klein, U. 1998, ApJ, 502L, 143

\bibitem[Walter et al.(2002)]{wa02} Walter, F., Weiss, A., \& Scoville, N. 2002, ApJ, 580, L21

\bibitem[Wang(1995)]{w95} Wang, B. 1995, ApJ, 444, 590

\bibitem[Wang et al.(2002)]{w02} Wang, Q. D., Gotthelf, E. V., \& Lang, C. C. 2002, Nature, 415, 148

\bibitem[White et al.(1991)]{w91} White, R. L., Becker, R. H., \& Helfand, D. J. 1991, ApJ, 371, 148

\bibitem[Wieringa et al.(1993)]{w93} Wieringa, M. H., de Bruyn, A. G., Jansen, D., Brouw, W. N., \& Katgert, P. 1993, A\&A, 268, 215

\bibitem[Wilson et al.(1982)]{w82} Wilson, T. L., Ruf, K., Walmsley, C. M., Martin, R. N., Batrla, W., \& Pauls, T. A. 1982, A\&A, 115, 185

\bibitem[Yang \& Skillman(1993)]{y93} Yang, H. \& Skillman, E. D. 1993, AJ, 106, 1448

\bibitem[Yusef-Zadeh(1986)]{y86} Yusef-Zadeh, F. 1986, Ph.D thesis, Columbia University

\bibitem[Yusef-Zadeh(2003)]{y03} ------ 2003, ApJ, 598, 325

\bibitem[Yusef-Zadeh \& Morris(1987a)]{y87} Yusef-Zadeh, F. \& Morris, M. 1987, ApJ, 320, 545

\bibitem[Yusef-Zadeh \& Morris(1987b)]{y87b} Yusef-Zadeh, F. \& Morris, M. 1987, ApJ, 322, 721

\bibitem[Yusef-Zadeh \& Morris(1988)]{y88} ------ 1988, ApJ, 329, 729

\bibitem[Yusef-Zadeh et al.(2002)]{y02} Yusef-Zadeh, F., Law, C., Wardle, M., Wang, Q. D., Fruscione, A., Lang, C. C., \& Cotera, A. 2002, ApJ, 570, 665

\bibitem[Yusef-Zadeh et al.(1984)]{y84} Yusef-Zadeh, F., Morris, M., \& Chance, D. 1984, Nature, 310, 557

\bibitem[Yusef-Zadeh et al.(2004)]{y04} Yusef-Zadeh, F., Hewitt, J., \& Cotton, W.  2004, ApJS, 155, 421

\bibitem[Yusef-Zadeh et al.(1997)]{y97} Yusef-Zadeh, F., Wardle, M., \& Parastaran, P. 1997, ApJ, 475L, 119

\bibitem[Yusef-Zadeh et al.(1995)]{y95} Yusef-Zadeh, F., Uchida, K. I., \& Roberts, D. A. 1995, Science, 270, 1801

\bibitem[Yusef-Zadeh et al.(2003)]{yu03} Yusef-Zadeh, F., Wardle, M., Rho, J., \& Sakano, M. 2003, ApJ, 585, 319

\bibitem[Yusef-Zadeh et al.(2006)]{y06} Yusef-Zadeh, F., et al. 2006, ApJ, 644, 198

\bibitem[Zhao et al.(1992)]{z92} Zhao, J.-H., et al. 1992, Science, 255, 1538

\end{thebibliography}

